Flexible Computational Pipelines for Robust Abstraction-Based Control Synthesis

Successfully synthesizing controllers for complex dynamical systems and specifications often requires leveraging domain knowledge as well as making difficult computational or mathematical tradeoffs. This paper presents a flexible and extensible framework for constructing robust control synthesis algorithms and applies this to the traditional abstraction-based control synthesis pipeline. It is grounded in the theory of relational interfaces and provides a principled methodology to seamlessly combine different techniques (such as dynamic precision grids, refining abstractions while synthesizing, or decomposed control predecessors) or create custom procedures to exploit an application's intrinsic structural properties. A Dubins vehicle is used as a motivating example to showcase memory and runtime improvements.

==> ops.tex <==
\subsection{Atomic and Composite Operators} \label{sec:core}


%\begin{table}
%\centering
%\begin{tabular}{|c|c|c|}
%\hline 
%Atomic Operators  & Predicate  & Interface \\
%  & Representation & Signature \\ \hline
%$\ohide(w,F(i,o))$ & $\equant{w}F$ & $(i, o \setminus w)$ \\ \hline
%$\ihide(w,F(i,\emptyset))$ & $\equant{w}F$  & $(i \setminus w, \emptyset)$ \\ \hline
%$\comp(F_1(i_1,o_1), F_2(i_2, o_2))$ & $F_1 \AND F_2 \AND \uquant{io_{12}} (F_1 \implies \NB{F_2})$ & $((i_1 \cup i_2) \setminus io_{12}, o_1 \cup o_2)$  \\
%& where $io_{12} = i_2 \cap o_1$ &  \\ \hline
%$\refine(F_1(i,o),F_2(i,o))$ & $(\NB{F_1} \OR \NB{F_2}) $ & $(i,o)$\\
%& $\AND (\NB{F_1} \implies F_1) \AND (\NB{F_2} \implies F_2) $ &  \\ \hline 
%\end{tabular}
%\end{table}

Operators are used to manipulate interfaces by taking interfaces and variables as inputs and yielding another interface.
%Operators can also be composed to construct new ones.
We will show how the controlled predecessor $\CPRE(\cdot)$ in \pref{eqn:origcpre} can be constructed by composing operators appearing in \cite{tripakis2011theory} and one additional one.
%\todo{Control synthesis toolboxes temporally discretize continuous time systems by fixing a sampling time step and imposing controllable inputs to have a zero order hold \cite{gunther2}.}
The first, output hiding, removes interface outputs.%, such as those that were shared internal variables before composition relabeled them as outputs.
\begin{definition}[Output Hiding \cite{tripakis2011theory}] \label{def:varhiding}
Output hiding operator $\ohide(w, F)$ over interface $F(\II, \OO)$ and outputs $w$ yields an interface with signature $(\II,\OO \setminus w)$.
\begin{align}
\ohide(w, F) = \equant{w}F
\end{align}
\end{definition}
Existentially quantifying out $w$ ensures that the input-output behavior over the unhidden variables is still consistent with potential assignments to $w$.
The operator $\NB{\cdot}$ is a special variant of $\ohide(\cdot)$ that hides all outputs, yielding a sink encoding all non-blocking inputs to the original interface.
%In the context of \Cref{fig:cpre}, $\ohide(x^+, \comp(F,Z))$ is a sink interface $(x \cup u, \emptyset)$ signifying the set of all state-input pairs for which $Z$ will be satisfied under dynamics $F$. 

\begin{definition}[Nonblocking Inputs Sink] \label{def:NB}
Given an interface $F(\II,\OO)$, the nonblocking operation \NB{F} yields a sink interface with signature $(i, \emptyset)$ and predicate $\NB{F} = \equant{\OO}F$.
%\begin{align}
%\NB{F} = \equant{\OO}F.
%\end{align}
If $F(i, \emptyset)$ is a sink interface, then $\NB{F} = F$ yields itself. If $F(\emptyset, o)$ is a source interface, then $\NB{F} = \false$ if and only if $F \lequiv \false$; otherwise $\NB{F} = \true$. 
\end{definition}


The interface composition operator takes multiple interfaces and ``collapses" them into a single input-output interface. It can be viewed as a generalization of function composition in the special case where each interface encodes a total function (i.e., deterministic output and inputs never block).
%\begin{figure}
%\centering
%\includegraphics[width=.5\columnwidth]{figs/cpresequence.png}
%\caption{\small Control predecessor as a sequence of interface operations. Interface $F(x \cup u, x^+)$ represents system dynamics and sink interface $Z(x^+, \emptyset)$ represents a target set of states. \todo{Pseudocode in python}} \label{fig:cpre}
%\end{figure}


\newcommand\IO[1]{io_{#1}}
\begin{definition}[Interface Composition \cite{tripakis2011theory}] 
Let $F_1(\II_1, \OO_1)$ and $F_2(\II_2, \OO_2)$ be interfaces with disjoint output variables $\OO_1 \cap \OO_2 \sequiv \emptyset$ and $\II_1 \cap \OO_2 \sequiv \emptyset$ which signifies that $F_2$'s outputs may not be fed back into $F_1$'s inputs.
Define new composite variables
\begin{align}
\IO{12} &\sequiv \OO_1 \cap \II_2\\
\II_{12} &\sequiv (\II_1 \cup \II_2) \setminus \IO{12} \\
\OO_{12} &\sequiv \OO_1 \cup \OO_2. %\cup \IO{12}
\end{align}
Composition $\comp(F_1, F_2)$ is an interface with signature $(i_{12}, o_{12})$ and predicate
\begin{align}
F_1 \AND F_2  \AND \uquant{\OO_{12}}(F_1 \implies \NB{F_2}). \label{eq:compositionpredicate}
\end{align}
Interface subscripts may be swapped if instead $F_2$'s outputs are fed into $F_1$.
\label{def:modcomposition}
\end{definition}

Interfaces $F_1$ and $F_2$ are composed in parallel if $io_{21} \sequiv \emptyset$ holds in addition to $io_{12} \sequiv \emptyset$. \Cref{eq:compositionpredicate} under parallel composition reduces to $F_1 \AND F_2$ (Lemma 6.4 in \cite{tripakis2011theory}) and $\comp(\cdot)$ is commutative and associative. If $io_{12} \not\equiv \emptyset$, then they are composed in series and the composition operator is only associative. 
%\Cref{fig:cpre} depicts the series composition of $F$ and $Z$.
Any acyclic interconnection can be composed into a single interface by systematically applying \Cref{def:modcomposition}'s binary composition operator.

Non-deterministic outputs are interpreted to be \textit{adversarial}.
Series composition of interfaces has a built-in notion of robustness to account for $F_1$'s non-deterministic outputs and blocking inputs to $F_2$ over the shared variables $io_{12}$.
%The last term in \Cref{eq:compositionpredicate} is a predicate over the expanded input set $i_{12}$ and deals with blocking behaviors under series composition.
%The series composition changes the role of variables $io_{12} \subseteq i_2$ from inputs to outputs.
The term $\uquant{\OO_{12}}(F_1 \implies \NB{F_2})$ in \Cref{eq:compositionpredicate} is a predicate over the composition's input set $i_{12}$. It ensures that if a potential output of $F_1$ may cause $F_2$ to block, then $\comp(F_1, F_2)$ must preemptively block.
%\begin{align}
%\NB{\comp(F_1, F_2)} = \equant{o_{12}} (F_1 \AND F_2) \AND \uquant{o_{12}} (F_1 \implies \NB{F_2})
%\end{align}


%This is one of many instances of composite operators being constructed from smaller primitives.
%Applying a nonblocking operator on every single output yields a sink interface that encodes the interface's nonblocking inputs.
The final atomic operator is input hiding, which may only be applied to sinks. If the sink is viewed as a constraint, an input variable is ``hidden" by an angelic environment that chooses an input assignment to satisfy the constraint. This operator is analogous to projecting a set into a lower dimensional space.
\begin{definition} [Hiding Sink Inputs]
Input hiding operator $\ihide(w,F)$ over sink interface $F(i, \emptyset)$ and inputs $w$ yields an interface with signature $(i \setminus w, \void)$.
\begin{align}
\ihide(w, F) = \equant{w} F
\end{align}
%yields an interface with signature . 
\end{definition}
Unlike the composition and output hiding operators, this operator is not included in the standard theory of relational interfaces \cite{tripakis2011theory} and was added to encode a controller predecessor introduced subsequently in \Cref{eqn:compositecpre}.

%\begin{table}
%\centering
%\begin{tabular}{|c|c|c|}
%\hline
%Composite  & Atomic  & Interface \\ 
%Operators& Representation & Signature \\ \hline 
%$\NB{F(i,o)}$ & $\equant{o}F$  & $(i,\emptyset)$ \\ \hline
%$\CPRE(F(x \cup u, x^+),Z(x^+, \emptyset))$ & $\ihide(u, \ohide(x^+, \comp(F,Z)))$ & $(x, \emptyset)$ \\ \hline
%$\incoarsen(F(i,o), Q(\abs i, i))$ & $\ohide(i, \comp(Q(\abs i, i), F) )$ & $(\abs i,o)$ \\ \hline
%$\outcoarsen(F(i,o), Q(o, \abs o))$ & $ \ohide(o, \comp( F, Q(o, \abs o)))$ & $(i, \abs o)$ \\ \hline
%\end{tabular}
%\end{table}

\subsection{Constructing Control Synthesis Pipelines}

The robust controlled predecessor (\ref{eqn:origcpre}) can be expressed through operator composition.
%Note that operator composition and interface composition are distinct within this framework.
\begin{proposition} \label{prop:cpreop}
The controlled predecessor operator \pref{eqn:compositecpre} % $\CPRE(F,Z)$ 
%\pref{eqn:compositecpre}.
yields a sink interface with signature $(x, \emptyset)$ and predicate equivalent to the predicate in \pref{eqn:origcpre}.
\begin{align}
\CPRE(F, Z) &= \ihide(u, \ohide(x^+, \comp(F,Z))). \label{eqn:compositecpre}
\end{align}
\end{proposition}
\ifcav
The simple proof is provided in the extended version.
\else
\begin{proof}
Applying the definitions of $\comp$, $\ihide$, and $\ohide$ yields the expression 
\begin{align}
\equant{u}\equant{x^+}(F \AND Z \AND \uquant{x^+}(F \implies Z)))
\end{align}
One can safely move the $\equant{x^+}$ inside the parenthesis because $\uquant{x^+}(F \implies Z)$ is a predicate that is independent of $x^+$, yielding
\begin{align}
\equant{u}(\equant{x^+}(F \AND Z) \AND \uquant{x^+}(F \implies Z)))
\end{align}
To show equivalence of the above expressions with \Cref{eqn:origcpre}, we simply need to show equivalence of the following two predicates that depend on $x$ and $u$:
\begin{align}
\equant{x^+}(F \AND Z) \AND \uquant{x^+}(F \implies Z) \label{eqn:xu1}\\
\equant{x^+} F \AND \uquant{x^+}(F \implies Z). \label{eqn:xu2}
\end{align}
It is easy to see that \pref{eqn:xu1} implies \pref{eqn:xu2} because $\equant{x^+}(F\AND Z)$ implies $\equant{x^+}F$. To show the reverse, suppose \pref{eqn:xu2} is satisfied for a pair $x$ and $u$. Any $x^+$ chosen to satisfy $\equant{x^+}F$ must also satisfy the constraint imposed by the sink $Z$. Otherwise, the clause $\uquant{x^+}(F \implies Z)$ would be violated, contradicting satisfaction of \pref{eqn:xu2}. Therefore, \pref{eqn:xu1} and \pref{eqn:xu2} are equivalent which completes the proof.
\end{proof}
\fi
 %provided in \Cref{cprepropproof} of the appendix.
\Cref{prop:cpreop} signifies that controlled predecessors can be interpreted as an instance of robust composition of interfaces, followed by variable hiding.
It can be shown that $\code{safe}(F,Z, S) = \comp(\CPRE(F, Z), S)$ because $S(x, \emptyset)$ and $\CPRE(F, Z)$ would be composed in parallel. \footnote{Disjunctions over sinks are required to encode $\code{reach}(\cdot)$. This will be enabled by the shared refinement operator defined in \Cref{def:refinement}.}

%\begin{wrapfigure}{r}{2.5in}
\begin{figure}[!t]
\centering
\includegraphics[width=.5\columnwidth]{nestedsafety.png}
%\includegraphics[width=.8\columnwidth]{figs/cprepipeline.png}
\caption{\small Safety control synthesis iteration \pref{safegame:iter} depicted as a sequence of sink interfaces.} \label{fig:cprepipeline}
%\end{wrapfigure}
\end{figure}
\Cref{fig:cprepipeline} shows a visualization of the safety game's fixed point iteration from the point of view of relational interfaces.
Starting from the right-most sink interface $S$ (equivalent to $Z_0$) the iteration \pref{safegame:iter} constructs a sequence of sink interfaces $Z_1, Z_2,...$ encoding relevant subsets of the state space.
The numerous $S(x, \emptyset)$ interfaces impose constraints and can be interpreted as monitors that raise errors if the safety constraint is violated.
%The controlled predecessor $\CPRE(F,Z)$ collapses $Z_0$ and $F$ down into another sink interface $Z_1$. This sink, when composed with $F$, yields another sink interface over the variables $x \cup u$.

\subsection{Modifying the Control Synthesis Pipeline}

\Cref{eqn:compositecpre}'s definition of $\CPRE(\cdot)$ is oblivious to the domains of variables $x,u$, and $x^+$. This generality is useful for describing a problem and serving as a blank template.
%The most common reason to modify the pipeline is to computational tractability.
Pipeline modifications allow a user to inject implicit preferences into a problem and reduce computational bottlenecks or to refine a solution.
Whenever problem structure exists, modifications refine the general algorithm into a form that reflects the specific problem instance.
%They also can explicitly capture structure, whenever it exists, and mold an algorithm to reflect it.
%alternatively to inject it.
%Only when a specific structural property in the dynamics or the specification.
%\todo{Make more concrete. Domain specific issues like termination. Structure is often domain specific. Modifications are domain specific.}
%The tools in  implement the abstraction and synthesis steps; some are augmented with techniques to mitigate the computational burdens of synthesizing controllers for systems with high dimensional continuous state spaces.
The subsequent sections apply this philosophy to the abstraction-based control techniques from \Cref{subsec:abcs}:
\begin{itemize}
\item \Cref{sec:refinementpo}: Coarsening interfaces reduces the computational complexity of a problem by throwing away fine grain information. The synthesis result is conservative but the degree of conservatism can be modified.
\item \Cref{sec:abs}: Refining interfaces decreases result conservatism. Refinement in combination with coarsening allows one to dynamically modulate the complexity of the problem as a function of multiple criteria such as the result granularity or minimizing computational resources. 
\item \Cref{sec:decomppre}: If the dynamics or specifications are decomposable then the control predecessor operator can be broken apart to refect that decomposition.
\end{itemize}
These sections do more than simply reconstruct existing techniques in the language of relational interfaces. 
They uncover some implicit assumptions in existing tools and either remove them or make them explicit.
Minimizing the number of assumptions ensures applicability to a diverse collection of systems and specifications and compatibility with future algorithmic modifications.
%Restricting one's self to a simple, yet powerful collection of well-understood primitives gives a safe and disciplined foundation for exploring future algorithmic modifications.

%\todo{Coarsening during synthesis. Computationally constrained. BDDs and finite. Decomposed predecessor}

%\todo{Better to compute an underapproximation than to fail to compute an exact solution.}
%In the context of controller synthesis,
%Whenever computing $\CPRE(F,Z)$ is intractable, one may instead decide to discard fine grain information and instead computing over a simpler model
%\begin{align}
%\CPRE(\coarsen(F),\coarsen(Z))
%\end{align}
%at the cost of yielding a conservative result. On the other hand, if $\CPRE(F,Z)$'s result is deemed unsatisfactory or too conservative, then the model  can be refined with additional information $K$ and 
%\begin{align}
%\CPRE(\refine(F, K),Z)
%\end{align}
%yields a more precise result.

%Input mask and output havoc are operators that are used to focus the synthesizer to specific sub-regions and ignore others.
%Like the coarsening operator, both input mask and output havoc operators make an interface more abstract according to the refinement relation and are useful for making controller synthesis more tractable. 
%
%Input masking causes a subset of input assignments to block. 
%\begin{definition} Let $I$ be a predicate over the same domain as $M$'s inputs.
%\begin{align}
%\code{mask}(M, I) = I \AND M 
%\end{align}
%\end{definition}
%
%This operator is commonly used if it is known that the system must satisfy a safety constraint. All known unsafe states can be removed from the system description because... 
%
%
%Output havoc is a similar operator that increases output non-determinism whenever an output exists.
%\begin{definition}
%\begin{align}
%\code{havoc}(M, O) = ( \equant{o}. M \AND O) \OR M
%\end{align}
%\end{definition}
%The first term is the set of inputs for where there exists an output satisfying $O$. The disjunction with the original interface permits all outputs. 


%\todo{Pseudo code here for cpre.  Start out with a python function with the declared synthesis game. Then talk about different optimizations to do.}








